Naturalistic Head Motion Generation from Speech

Synthesizing natural head motion to accompany speech for an embodied conversational agent is necessary for providing a rich interactive experience. Most prior works assess the quality of generated head motion by comparing them against a single ground-truth using an objective metric. Yet there are many plausible head motion sequences to accompany a speech utterance. In this work, we study the variation in the perceptual quality of head motions sampled from a generative model. We show that, despite providing more diverse head motions, the generative model produces motions with varying degrees of perceptual quality. We finally show that objective metrics commonly used in previous research do not accurately reflect the perceptual quality of generated head motions. These results open an interesting avenue for future work to investigate better objective metrics that correlate with human perception of quality.

==> tables/table_2.tex <==
\begin{table}[t]
  \centering
\resizebox{\columnwidth}{!}{
  \begin{tabular}{lcccc}
    \toprule
    \textbf{} & \textbf{Estimate} &  \textbf{Std. Error}  &  $\mathbf{z}$ &  $\mathbf{p}$\\
    \midrule
    Deterministic       & $0.22$ & $0.14$ & $1.53$ & $0.12$\\
    Group $1$       & $0.26$ & $0.12$ & $2.1$ & $0.03$\\
    Group $2$      & $0.5$ & $0.12$ & $4.04$ & $<0.0001$\\
    Group $3$       & $0.7$ & $0.12$ & $5.6$ & $<0.0001$\\
    Group $4$      & $0.91$ & $0.12$ & $7.24$ & $<0.0001$\\
    Group $5$        & $1.00$ & $0.13$ & $7.83$ & $<0.0001$\\
    Group $6$       & $1.21$ & $0.13$ & $9.51$ & $<0.0001$\\
    Group $7$        & $1.31$ & $0.13$ & $10.18$ & $<0.0001$\\
    Group $8$       & $1.58 $& $0.13$ & $12.03$ & $<0.0001$\\
    Group $9$       & $1.75$ & $0.13$ & $13.18$ & $<0.0001$\\
    Group $10$       & $2.18$ & $0.14$ & $15.7$ & $<0.0001$\\
    \bottomrule
  \end{tabular}
  }
  \caption{Comparison of the head motions produced by the deterministic and non-deterministic models to the ground-truth. Lack of significance indicates no preference between the generated and ground-truth head-motions. Positive estimates indicate a preference for the ground-truth head-motion. Negative estimates indicate a preference for the generated head-motion. See Section~\ref{sec:perceptual_quality} for model details.}
  \label{tab:regression_results1}
\end{table}


==> tables/table_3.tex <==
\begin{table}[t]
  \centering
  \begin{tabular}{lcc}
    \toprule
    \textbf{} & \textbf{Pearson coefficient} &  $\mathbf{p}$\\
    \midrule
    MAE       & $-0.38$ & $<0.001$\\
    DTW       & $-0.39$ & $<0.001$\\
    FD       & $-0.38$ & $<0.001$\\
   % VAR       & $0.03$ & $0.32$ \\
    \bottomrule
  \end{tabular}
  \caption{Correlation between objective measures and perceptual quality. MAE, DTW, and FD are the mean absolute error, dynamic time warping distance, and the Frechet distance, respectively.}
  \label{tab:correlations}
\end{table}


